Best-of-Both-Worlds Policy Optimization for CMDPs with Bandit Feedback

We study online learning in constrained Markov decision processes (CMDPs) in which rewards and constraints may be either stochastic or adversarial. In such settings, Stradi et al.(2024) proposed the first best-of-both-worlds algorithm able to seamlessly handle stochastic and adversarial constraints, achieving optimal regret and constraint violation bounds in both cases. This algorithm suffers from two major drawbacks. First, it only works under full feedback, which severely limits its applicability in practice. Moreover, it relies on optimizing over the space of occupancy measures, which requires solving convex optimization problems, an highly inefficient task. In this paper, we provide the first best-of-both-worlds algorithm for CMDPs with bandit feedback. Specifically, when the constraints are stochastic, the algorithm achieves $\widetilde{\mathcal{O}}(\sqrt{T})$ regret and constraint violation, while, when they are adversarial, it attains $\widetilde{\mathcal{O}}(\sqrt{T})$ constraint violation and a tight fraction of the optimal reward. Moreover, our algorithm is based on a policy optimization approach, which is much more efficient than occupancy-measure-based methods.

==> Adversarial_Setting.tex <==
\section{Adversarial setting}

\begin{restatable}{theorem}{advconst}
	When Condition~\ref{ass:rhoassumption} holds and the constraints are adversarial the following results hold.\\
	In case of adversarial rewards, with probability at least $1-13\delta$ and in case of stochastic rewards, with probability at least $1-14\delta$:
	
	\begin{equation*}
		\sum_{t=1}^T r_t^\top q_t \ge \Omega\left(\frac{\rho}{\rho+H}\cdot\text{OPT}_{\overline r, \overline G}\right), \quad V_T \le \BigOL{\Lambda\sqrt{T}}
	\end{equation*}
\end{restatable}

\subsection{Weaker Baseline}

\begin{restatable}{theorem}{weakbasecond}
	If Condition \ref{ass:rhoassumption} holds, then the constraints violation and the regret computed with respect to an optimal policy that respect the constraints at each episode can be bounded in the following way. 
	In case of adversarial constraints, with adversarial rewards it holds with probability at least $1-12\delta$, and with stochastic rewards it holds with probability at least $1-13\delta$:
	\begin{equation*}
		R_T \le \BigOL{\Lambda\sqrt{T}}, \quad V_T \le \BigOL{\Lambda\sqrt{T}}
	\end{equation*}
\end{restatable}

\begin{restatable}{theorem}{weakbasenocond}
	If Condition \ref{ass:rhoassumption} does not hold, then the constraints violation and the regret computed with respect to an optimal policy that respects the constraints at each episode can be bounded in the following way. 
	In case of adversarial  constraints, with adversarial rewards it holds with probability at least $1-11\delta$ and with stochastic rewards it holds with probability at least $1-12\delta$:
	\begin{equation*}
		R_T \le \BigOL{T^{\nicefrac{3}{4}}}, \quad V_T \le \BigOL{T^{\nicefrac{3}{4}}} 
	\end{equation*}
\end{restatable}

==> Stochastic_Setting.tex <==
\section{Stochastic Setting}
In this section we study the performance of the algorithm in case of stochastic constraints. In general thank to the no-interval regret property of the primal and dual algorithm, in addition to the employ of the lagrangian function, we prove that the orders of both the regret and the constraints violation are the product of a sublinear factor of order $\BigOL{T^{\nicefrac{1}{2}}}$ generated by the primal regret, the dual regret and the employ of Azuma-Hoeffding inequality that accounts for the difference between the empirical observed mean and the theoretical mean of the distribution for the constraints and, in case of stochastic rewards, also of the rewards, and the maximum value taken over all episode of the module $1$ of the lagrangian multipliers, \emph{i.e.} $\max_{t \in [T]}\lVert \lambda_t \rVert_1$.
When Condition~\ref{ass:rhoassumption} holds, the lagrangian multipliers are nicely bounded by $\Lambda$ leading to the following result.
\begin{restatable}{theorem}{stocconstcond}
	\label{theo: assumption + stoch cost}
	Suppose Condition~\ref{ass:rhoassumption} holds, in case of stochastic constraints the following results also hold.
	If the rewards are stochastic with probability at least $1-14\delta$ and if the rewards are adversarial with probability at least $1-13\delta$ it holds:
	\begin{equation*}
		R_T \le \BigOL{\Lambda\sqrt{T}} \quad \land \quad V_T \le \BigOL{\Lambda\sqrt{T}}
	\end{equation*}
\end{restatable}
Finally when the Condition~\ref{ass:rhoassumption} does not hold, we can still use the bounds of the dual space, and therefore the Lagrangian multipliers are bounded by the quantity $mT^{\nicefrac{1}{4}}$, leading to the following result.
\begin{restatable}{theorem}{stocconstnocond}
	\label{theo: not cond stoc constr}
	When Condition~\ref{ass:rhoassumption} does not hold, whenever the constraints are stochastic, Algorithm \ref{Alg: total} achieves the following guarantees.
	In case of stochastic rewards  with probability at least $1-11\delta$ and in case of adversarial rewards with probability at least $1-10\delta$ it holds:
	\begin{equation*}
		R_T \le \BigOL{T^{\nicefrac{3}{4}}}, \quad V_T \le \BigOL{T^{\nicefrac{3}{4}}}
	\end{equation*}
\end{restatable}
